Adaptive Rejection of Periodic Disturbances Acting on Linear Systems with Unknown Dynamics

This paper proposes a novel direct adaptive control method for rejecting unknown deterministic disturbances and tracking unknown trajectories in systems with uncertain dynamics when the disturbances or trajectories are the summation of multiple sinusoids with known frequencies, such as periodic profiles or disturbances. The proposed algorithm does not require a model of the plant dynamics and does not use batches of measurements in the adaptation process. Moreover, it is applicable to both minimum and non-minimum phase plants. The algorithm is a "direct" adaptive method, in the sense that the identification of system parameters and the control design are performed simultaneously. In order to verify the effectiveness of the proposed method, an add-on controller is designed and implemented in the servo system of a hard disk drive to track unknown nano-scale periodic trajectories.

==> apndx-proof-directadaptive.tex <==
\section{Proof of Theorems }
We use the method of analysis of stochastic recursive
algorithms discussed in \cite{ljung1977analysis} to study the
convergence and asymptotic behavior of the proposed adaptive algorithm with
the update rule given in \eqref{eq:paa}.
The key idea is that a differential equation counterpart 
for \eqref{eq:paa} is derived and it is shown that
the only convergence point of \eqref{eq:paa} is the 
stable equilibrium of this differential equation.
Moreover, it is shown that the estimated parameters
 converge with probability one to this equilibrium under
some mild assumptions on the excitation signal power or initial 
values of parameters.

\subsection{Preliminaries}
A general recursive algorithm can be formalized as
\begin{align}\label{eq:paa-general}
\hat{\Theta}(k)=\hat{\Theta}(k-1)+ \gamma(k)Q(k;\hat{\Theta}(k-1), \Phi(k))
\end{align}
where $\hat{\Theta}(k)\in \R^n$ is a sequence of $n$-dimensional column vectors
referred as  ``the estimates''. In our particular recursive algorithm, they stand for
the parameters of system dynamics in conjunction with the parameters that determine the adaptive control law.
$\gamma(k)$ is assumed to be
a sequence of positive scalars. The $m$-dimensional vector
$\Phi(k)$ is an observation obtained at time $k$ which is usually called the ``regressor''. The information
contained in $\Phi(k)\in \R^m$ sequence cause $\hat{\Theta}(k-1)$ to be updated.
The map $Q(.;.,.)$ from $R\times R^n \times R^m$ into $R^n$ is a
deterministic function with some regularity conditions that 
guarantee the convergence of the adaptive algorithm to 
some ``desired'' points that will be discussed later. 
%From the above equation it can be inferred that 
%$Q(.;.,.)$ together with the choice
%of the ``gain'' sequence $\gamma(.)$ determine entirely the
%algorithm.

The regressor vector $\Phi(k)$ is, in general, a function of the
previous measurements (when the system has memory), the 
previous estimates (when the estimates define an adaptive control law),  
and the inputs to the system (all other control signals and noises).
A very broad class of update rules, as of ours, can be realized by a 
time varying linear system
\begin{align*}
\Phi(k)= A_{\Phi}(\hat{\Theta}_{k-1}) \Phi(k-1) + B_{\Phi}(\hat{\Theta}_{k-1}) U(k)
\end{align*}
where $A_{\Phi}$ and $B_{\Phi}$ are $m\times m $ and $m\times r$ matrix functions and $U(k)\in \R^r$ stands for all control signals and noises entering the system.

In a stochastic framework, $Q(k;\hat{\Theta}(k-1), \Phi(k))$ is a random variable. This implies that
convergence can take place only if the noise is rejected by paying less
attention to the observations as time passes, i.e. by letting
\begin{align*}
\gamma(k)\rightarrow 0 \qquad \text{as}~~ k\rightarrow \infty.
\end{align*}
However, this is not feasible when the actual (system) parameters are time-varying, as in 
tracking problems. 
For such problems, $\gamma(k)$ can tend to very small, but still positive, values and 
the analysis carried out in this section will give some insights regarding the
algorithm behavior.

The estimated parameters and the regressor in our adaptive algorithm are
	\begin{align*}
		&\hat{\Theta}(k):=\begin{bmatrix} \tha_A(k) \\ \tha_B(k) \\ \tha_C(k) \\ \tha_M(k)  \\ \text{col}\left[F(k)\right] \\ f(k) \end{bmatrix}
		%
		&\Phi(k):= 
		\left[\begin{array}{c}
		\phi_{e}(k) \\ \hdashline u(k) \\ \phi_u(k) \\ \hdashline {\bar{w}}(k) \\\phi_{\bar{w}}(k) \\ \hdashline \phi_{\epsilon}(k) \\\hdashline \phi_R(k) \\\hdashline \phi_{ u_{A}}(k)
		\end{array} \right].
	\end{align*}
where $\text{col}[x]$ of a matrix $x$ refers to a vector created by stacking the columns of matrix $x$.
The $A_{\Phi}$ and $B_{\Phi}$ matrix functions can be written as

	\begin{widetext}
		\begin{align}\label{eq:A}
		A_{\Phi}(\hat{\Theta}_{k-1}):=
		{\tiny
			\left[\begin{array}{cccccccc}
			%
			\theta_A^T  & \begin{bmatrix} 0 & \theta_B^T \end{bmatrix} & \begin{bmatrix} 0 & \theta_C^T  \end{bmatrix}& 0_{n_A} & \theta_R^T & \theta_B^T \\ 
			\begin{bmatrix} I_{n_A-1} & 0 \end{bmatrix} &0 &0 &0 &0 &0 \\\hdashline 
			%
			0 & \begin{bmatrix} 0 & 0\\I_{n_A} & 0   \end{bmatrix} &0 &0 &0 &0 \\ \hdashline
			%
			0 & 0  & \begin{bmatrix} 0 & 0 \\I_{n_A} & 0  \end{bmatrix} & 0 &0 &0 \\ \hdashline
			%
			\hat{\theta}_A^T(k-1)& \begin{bmatrix} 	0 & \hat{\theta}_B^T(k-1) \end{bmatrix} &0 &\hat{\theta}_C^T(k-1) &\hat{\theta}_M^T(k-1) &0 \\
			0 & 0 & 0 & \begin{bmatrix} I_{n_A-1	} & 0  \end{bmatrix}  &0 &0 \\ \hdashline
			%
			0 & 0 & 0 & 0 & 0  &0 \\ \hdashline
			%
			0 &0 &0 &0 &\hat{\theta}_D^T(k-1) &0 \\ 
			0 & 0 & 0 &0 &0 &\begin{bmatrix} I_{n_A-1} & 0  \end{bmatrix} 
			\end{array} \right]}
		\end{align}
	\end{widetext}
% B
	\begin{align}\label{eq:B}
		B_{\Phi}(\hat{\Theta}_{k-1}):=
		\left[\begin{array}{ccc}
		0 & 0 &0\\\hdashline
		\begin{bmatrix} I \\ 0 \end{bmatrix} &0 &0\\\hdashline
		0& \begin{bmatrix} I \\ 0 \end{bmatrix} &0\\\hdashline
		0 & 0 &0\\\hdashline	
		0& 0& \begin{bmatrix} I \\ 0 \end{bmatrix} \\\hdashline
		0 & 0 &0	
		\end{array} \right]
		\end{align}
		and the input vector is
		\begin{align}\label{eq:U}
		U(k):=
		\left[\begin{array}{c}
		u(k)\\{\bar{w}}(k)\\\phi_R(k)
		\end{array} \right].
	\end{align}
The next part provides certain regularity
conditions on functions $Q$,  $A_{\Phi}$ and $B_{\Phi}$ as well as
driving ``input'' term $U$ to analyze the behavior of \eqref{eq:paa-general}.
Before that, we provide two Lemmas about Lipschitz continuity (LC) properties of real valued functions since these results will be used in the sequel. The proofs of both lemmas can be found in \cite{eriksson2013applied}.
\begin{lemma}[LC of product of functions]\label{lem:lcprod}
	$f(x)={f_1(x)}{f_2(x)}$ is Lipschitz continuous on a bounded set $I$ if $f_1(.)$ and $f_2(.)$ are individually Lipschitz continuous on the same set.
\end{lemma}
\begin{lemma}[LC of quotient of functions]\label{lem:lcquotient}
	$f(x)=\frac{f_1(x)}{f_2(x)}$ is Lipschitz continuous on a bounded set $I$ if $f_1(.)$ and $f_2(.)$ are individually Lipschitz continuous on the same set and there is a positive constant $m$ such that for any $x\in I$, $f_2(x)\ge m$.
\end{lemma}




\subsection{Regularity Conditions}
Three sets of regularity conditions are proposed in \cite{ljung1977analysis} to
analyze a recursive algorithm in the form of \eqref{eq:paa-general}.
The first two sets, referred as ``Assumptions A'' and ``Assumptions B'', 
consider $U(k)$ as a sequence of random variables and treat the algorithm in a stochastic framework.
In our method, the input signal $U(k)$ \eqref{eq:U} is consisted of stochastic and deterministic parts, e.g. $\Phi_R(k)$ is a known vector whereas $\bar{w}(k)$ is a random sequence.
The third set of assumptions referred as ``Assumptions C'' is more general and will be used here.
Let $\mathscr{D}_S(x)$ be the set of all $A_{\Phi}(x)$ that have all eigenvalues strictly inside the unit circle and 
let $\mathscr{D}_R$ be an open connected subset of $\mathscr{D}_S(x)$. ``Assumptions C'' in \cite{ljung1977analysis} are given in the following.

%=============================================================================================
\subsubsection{Assumptions C}\label{ass:c}
\begin{enumerate}
	\item \label{ass:c1} The function $Q\left(k,x,\phi\right)$ is Lipschitz continuous in $x$ and $\phi$. In other words, 
	$|Q\left(k,x_1,\phi_1\right)-Q\left(k,x_2,\phi_2\right)|<\mathscr{K}\left(x,\phi,\rho, \nu\right)\left\{|x_1-x_2|+|\phi_1-\phi_2|\right\}$ 
	for any $x_1$ and $x_2$ in $\mathscr{B}(x,\rho(x))$ ($\mathscr{B}(x,\rho)$ denotes a $\rho$-neighborhood of $x$) for some $\rho(x)>0$ where $x\in \mathscr{D}_R$. Moreover, $\phi_1$ and $\phi_2$ should be in $\mathscr{B}\left(\phi, \nu \right)$ for some $\nu \ge 0$.
	%
	\item \label{ass:c2} The matrix functions $A_{\Phi}(x)$ and $B_{\Phi}(x)$ are \lc\ in $x$.
	%
	\item \label{ass:c3} $z(k,\bar{x})$ as defined by $z(0,\bar{x})=0$ and 
		\begin{align}\label{eq:z}
			\begin{split}
			&z(k,\bar{x})=z(k-1,\bar{x})+\\
			&\qquad \quad \gamma(k)\left[Q(k,\bar{x},\bar{\phi}(k,\bar{x}))-z(k-1,\bar{x})\right] \\
			\end{split}
		\end{align}
	converges for all $\bar{x}\in\mathscr{D}_R$ as $k\rightarrow \infty$. Denote the limit by $\mathscr{F}(\bar{x})$.
	%
	\item \label{ass:c4} $k_v(k,\bar{x},\lambda,c)$ defined by $k_v(0,\bar{x},\lambda,c)=0$ and 
		\begin{align}\label{eq:kv}
		\begin{split}
			&k_v(k,\bar{x},\lambda,c) = k_v(k-1,\bar{x},\lambda,c)+\\
			&\quad \gamma(k) \left[\mathscr{K}\left(\bar{x},\bar{\phi}(k,\bar{x}),\rho(\bar{x}),\nu(k,\lambda,c)\right) \right. \\
			&\quad \quad 
			\cdot\left.
			\left(1+\nu(k,\lambda,c)\right)-k_\nu (k-1,\bar{x},\lambda,c)
			\right]
		\end{split}
		\end{align}
	converges to a finite limit as $k\rightarrow \infty$ for all $\bar{x}\in \mathscr{D}_R$, $\lambda<1$ and $c<\infty$.
	%
	\item \label{ass:c5} $\sum\limits_{k=1}^{\infty}\gamma(k)=\infty$.
	%
	\item \label{ass:c6} $\gamma(k)\rightarrow 0$ as $k\rightarrow \infty$.
\end{enumerate}


%\begin{assumption}	\label{ass:c1} The function $Q\left(k,x,\phi\right)$ is Lipschitz continuous in $x$ and $\phi$. In other words, 
%	$|Q\left(k,x_1,\phi_1\right)-Q\left(k,x_2,\phi_2\right)|<\mathscr{K}\left(x,\phi,\rho, \nu\right)\left\{|x_1-x_2|+|\phi_1-\phi_2|\right\}$ 
%	for any $x_1$ and $x_2$ in $\mathscr{B}(x,\rho(x))$ ($\mathscr{B}(x,\rho)$ denotes a $\rho$-neighborhood of $x$) for some $\rho(x)>0$ where $x\in \mathscr{D}_R$. Moreover, $\phi_1$ and $\phi_2$ should be in $\mathscr{B}\left(\phi, \nu \right)$ for some $\nu \ge 0$.
%\end{assumption}
%
%\begin{assumption}
% 	\label{ass:c2} The matrix functions $A_{\Phi}(x)$ and $B_{\Phi}(x)$ are \lc\ in $x$.
%\end{assumption}
%
%\begin{assumption}
%		\label{ass:c3} $z(k,\bar{x})$ as defined by $z(0,\bar{x})=0$ and 
%	\begin{align}\label{eq:z}
%	\begin{split}
%	&z(k,\bar{x})=z(k-1,\bar{x})+\\
%	&\qquad \quad \gamma(k)\left[Q(k,\bar{x},\bar{\phi}(k,\bar{x}))-z(k-1,\bar{x})\right] \\
%	\end{split}
%	\end{align}
%	converges for all $\bar{x}\in\mathscr{D}_R$ as $k\rightarrow \infty$. Denote the limit by $\mathscr{F}(\bar{x})$.
%\end{assumption}
%
%\begin{assumption}
%		\label{ass:c4} $k_v(k,\bar{x},\lambda,c)$ defined by $k_v(0,\bar{x},\lambda,c)=0$ and 
%	\begin{align}\label{eq:kv}
%	\begin{split}
%	&k_v(k,\bar{x},\lambda,c) = k_v(k-1,\bar{x},\lambda,c)+\\
%	&\quad \gamma(k) \left[\mathscr{K}\left(\bar{x},\bar{\phi}(k,\bar{x}),\rho(\bar{x}),\nu(k,\lambda,c)\right) \right. \\
%	&\quad \quad \cdot\left.
%	\left(1+\nu(k,\lambda,c)\right)-k_\nu (k-1,\bar{x},\lambda,c)
%	\right]
%	\end{split}
%	\end{align}
%	converges to a finite limit as $k\rightarrow \infty$ for all $\bar{x}\in \mathscr{D}_R$, $\lambda<1$ and $c<\infty$.
%\end{assumption}
%
%\begin{assumption}
%	\label{ass:c5} $\sum\limits_{k=1}^{\infty}\gamma(k)=\infty$.
%\end{assumption}
%
%\begin{assumption}
%	\label{ass:c6} $\gamma(k)\rightarrow 0$ as $k\rightarrow \infty$.
%\end{assumption}



\paragraph*{Assumption \ref{ass:c1}:} The function $Q(k;\hat{\Theta}(k-1),\Phi(k))$ in \eqref{eq:paa-general} in our algorithm is time invariant. We abuse the notation and use $Q(\hat{\Theta}(k-1),\Phi(k))$ in the sequel. This function can be written as
	\begin{align}
		\label{eq:Q}
		&Q\left(\hat{\Theta}(k-1), \Phi(k) \right):= \begin{bmatrix}Q_1(\hat{\Theta}(k-1), \Phi(k))\\Q_2(\hat{\Theta}(k-1), \Phi(k))\\Q_3(\hat{\Theta}(k-1), \Phi(k))\end{bmatrix}
	\end{align} 
where
	\begin{align}
		\label{eq:Q1}
		&Q_1(\hat{\Theta}(k-1), \Phi(k)):= \bm{cc} F^{-1}(k-1) & 0 \\ 0 & f^{-1}(k-1)I \mb
		\\ \notag
		&\qquad\quad  \cdot M_1 \Phi(k)\left(M_3^T \Phi(k)- M_2\hat{\Theta}^T(k-1)M_1\Phi(k)\right) 
		\\
		\label{eq:Q2}
		&Q_2(\hat{\Theta}(k-1), \Phi(k)):= \text{Col}\left\{ M_4   \Phi(k)\Phi^T(k) M_4^T - F(k-1) \right\}
		\\
		\label{eq:Q3}
		&Q_3(\hat{\Theta}(k-1), \Phi(k)):=  \Phi(k)^T M_5^T M_5 \Phi(k) - f(k-1)
	\end{align}
and the matrices $M_1$, $M_2$, $M_3$, $M_4$ and $M_5$ are defined as follows
	\begin{align}
	\notag 
	\phi(k):&=\begin{bmatrix}\phi_{e}(k) \\ \phi_u(k)\\ \phi_{\epsilon}(k) \\ \phi_R(k) \end{bmatrix}=\underbrace{\begin{bmatrix}
		\text{diag}\bk{ccccccc} I  & \begin{bmatrix} 0& I \end{bmatrix} & \begin{bmatrix} 0& I \end{bmatrix}&I  \kb
		& 0	\end{bmatrix}}_{M_1} \Phi(k)
	\\
	\notag
	\hat{\theta}(k):&=\begin{bmatrix}\tha_A(k)\\ \tha_B(k) \\ \tha_C(k) \\ \tha_M(k) \end{bmatrix} = \underbrace{\begin{bmatrix}
		I & 0
		\end{bmatrix}}_{M_2} \hat{\Theta}(k)
	\\
	%
	\notag
	{e}(k)&= \underbrace{\left[\begin{array}{cccccccc}
		%
		\theta_A^T  & \begin{bmatrix} 0 & \theta_B^T \end{bmatrix} & \begin{bmatrix} 0 & \theta_C^T  \end{bmatrix}& 0 & \theta_R^T & \theta_B^T 	\end{array} \right]}_{M_3^T} \Phi(k)
	\\
	%
	\notag
	\begin{bmatrix}\phi_{e}(k) \\ \phi_u(k)\\ \phi_{\epsilon}(k)  \end{bmatrix}&=\underbrace{\begin{bmatrix}
		\text{diag}\bk{ccccccc} I  & \begin{bmatrix} 0& I \end{bmatrix} &\begin{bmatrix} 0& I \end{bmatrix} \kb & 0
		\end{bmatrix}}_{M_4} \Phi(k) 
	\\
	\notag
	\phi_R(k) &=\underbrace{\bm{ccccccc} 0   &I & 0\mb}_{M_5} \Phi(k).
	\end{align}
The dimensions of identity and all zero matrices are omitted since they can be determined from the 
regressor and estimated parameters dimensions. 
Equation \eqref{eq:Q} shows that $Q(x,\phi)$ is Lipschitz continuous if $Q_1(x,\phi)$, $Q_2(x,\phi)$ and $Q_3(x,\phi)$ are all \lc. This can be shown by ``triangle inequality''
	$$|Q(x,\phi)|\le |Q_1(x,\phi)|+|Q_2(x,\phi)|+|Q_2(x,\phi)|$$
which implies that
	\begin{align*}
	&|Q(x_1,\phi_1) - Q(x_2,\phi_2) | \\ & \qquad \qquad \le \left(\mathscr{K}_1+\mathscr{K}_2+\mathscr{K}_3\right) \left\{|x_1-x_2|+|\phi_2 - \phi_2|\right\}
	\end{align*}
where $\mathscr{K}_1$, $\mathscr{K}_2$ and $\mathscr{K}_3$ are the Lipschitz constants of $Q_1(.,.)$, $Q_2(.,.)$ and $Q_3(.,.)$ in a bounded region of interest. With the same argument, we can claim that each $Q_i$ -- as a vector valued function -- is \lc\ if each of its individual components is \lc. Equations \eqref{eq:Q2} and \eqref{eq:Q3} show that $Q_2(.,.)$ and $Q_3(.,.)$ are always \lc\ by Lemma~\ref{lem:lcprod}. Moreover, $Q_1(.,.)$ is \lc\ as long as $F$ is non singular and $f$ is non zero. This can be shown by Lemma~\ref{lem:lcprod} and \ref{lem:lcquotient}, and the fact that matrix inversion incorporates determinants of sub-regions of the original matrix (i.e. cofactors) and inverse of the matrix determinant. It is clear that the cofactor elements are simply polynomials and thus \lc, and the inverse of the matrix determinant is \lc\ by Lemma~\ref{lem:lcquotient} as long as it is always nonsingular in $\mathscr{B}(x,\rho)\times \mathscr{B}(\phi,\nu)$.

\paragraph*{Assumption \ref{ass:c2}:} It is clear that $A_{\Phi}(\hat{\Theta})$ and $B_{\Phi}(\hat{\Theta})$ given by \eqref{eq:A} and \eqref{eq:B} are both (Lipschitz) continuous in $\hat{\Theta}$.

\paragraph*{Assumption \ref{ass:c3}:} By following the same approach as in the proof of Lemma 2 in \cite{ljung1977analysis}, we can show that when the following conditions are satisfied
\begin{enumerate}
	\item Assumption \ref{ass:c1} holds
	\item $\mathscr{K}$ in \ref{ass:c1} is \lc  ~in $\phi$ and $\nu$ 
		\begin{align*}
			&|\mathscr{K}\left(x,\phi_1,\rho,\nu_1 \right)
			-\mathscr{K}\left(x,\phi_2,\rho,\nu_2 \right)|
			\le  \\
			& \qquad \qquad \mathscr{H}\left(x,\phi,\rho,\nu,w \right)\left\{|\phi_1-\phi_2|+|\nu_1-\nu_2|\right\}
		\end{align*}
	for $\phi_1,\phi_2\in \mathscr{B}(\phi,w)$ and $\nu_1,\nu_2\in \mathscr{B}(\nu,w)$
	\item For all $x\in\mathscr{D}_R$, the functions $Q$, $\mathscr{K}$ and $\mathscr{H}$ have bounded $p$-moments for all $p>1$, $\lambda<1$ and $c<\infty$.
\end{enumerate}
we have
\begin{align}\label{eq:sumToExpect}
	\frac{1}{t}\sum\limits_{k=1}^{t} Q\left(\bar{x}, \bar{\phi}(k,\bar{x})\right) \rightarrow \frac{1}{t}\sum\limits_{k=1}^{t} \E \left[Q\left(\bar{x}, \bar{\phi}(k,\bar{x})\right)\right]
\end{align}
with probability one as $t\rightarrow \infty$.
We have already shown that \ref{ass:c1} holds and a \lc~ function $\mathscr{K}$ can be defined. The last condition holds as long as $|F(k)|$ and $|f(k)|$ are non-zero.
This expression \eqref{eq:sumToExpect} with \eqref{eq:z} when $\gamma(k)= 1/k$ imply
\begin{align}\label{eq:sumE}
	z(t,\bar{x})\rightarrow\frac{1}{t}\sum\limits_{k=1}^{t} \E \left[Q\left(\bar{x}, \bar{\phi}(k,\bar{x})\right)\right].
\end{align}
with probability one as $t\rightarrow \infty$.
Therefore, in order to show that regularity condition (C.3) is satisfied, it is enough to prove that the limit
$$\mathscr{F}(\bar{x})=\lim\limits_{t\rightarrow\infty}\frac{1}{t}\sum\limits_{k=1}^{t} \E \left[Q\left(\bar{x}, \bar{\phi}(k,\bar{x})\right)\right]$$
exists.

As we will show in the following part, the stochastic process $Q\left(\bar{x}, \bar{\phi}(k,\bar{x})\right)$ is cyclostationary and the limit is well defined. Here, we assume that the excitation signal is also periodic with contents focused at frequencies different than the periodic disturbance. We take $\bar{\Theta}\in \mathscr{D}_R$ which implies that $A_{\Phi}(\bar{\Theta})$ is stable (i.e. has all eigenvalues strictly inside the unit circle). Since $A_{\Phi}(\bar{\Theta})$ and $B_{\Phi}(\bar{\Theta})$ are time invariant, we can use superposition principle for this linear time invariant system and decompose the response $\Phi(k)=\Phi_s(k)+\Phi_d(k)$ into stochastic, $\Phi_s(k)$, and deterministic, $\Phi_d(k)$, parts
\begin{align}\label{eq:phid}
	\Phi_s(k) &= A_{\Phi}(\bar{\Theta}) \Phi_s(k-1) + B_{\Phi_s}(\bar{\Theta}) {\bar{w}}(k) \\ \label{eq:phs}
	\Phi_d(k) &= A_{\Phi}(\bar{\Theta}) \Phi_d(k-1) + B_{\Phi_d}(\bar{\Theta}) \begin{bmatrix} u(k) \\ \phi_R(k)	\end{bmatrix}
\end{align}
where $B_{\Phi_s}$ and $B_{\Phi_d}$ can be clearly found from \eqref{eq:B}. Note that when $u(k)$ is not periodic and rather it is wide-sense stationary the only required modification is to remove $u(k)$ from the input signal in \eqref{eq:phid} and instead append the input in \eqref{eq:phs} with $u(k)$. The rest of analysis will be very similar in this case.

Since $A_{\Phi}(\bar{\Theta})$ is stable, $\Phi_s(k)$ will converge to a zero mean stationary random vector, denoted by $\bar{\Phi}_s(k, \bar{\Theta})$, with bounded covariance and $\Phi_d(k)$ will converge to $\bar{\Phi}_d(k, \bar{\Theta})$ which is a periodic vector that contains sinusoids with the same frequencies as $\phi_R(k)$ and amplitudes/phase-lags that are related to the magnitude and phase of $$\left(e^{jw_i}I-A_{\Phi}(\bar{\Theta})\right)^{-1}B_{\Phi_d}(\bar{\Theta})e^{jw_i}.$$ 
Again, since $A_{\Phi}(\bar{\Theta})$ is stable, $\bar{\Phi}_d(k, \bar{\Theta})$ is bounded and it implies that ${\Phi}(k)$ will converge to $\bar{\Phi}(k, \bar{\Theta})=\bar{\Phi}_s(k, \bar{\Theta})+\bar{\Phi}_d(k, \bar{\Theta})$. We can now return to \eqref{eq:sumE} and show that 
\begin{align}\label{eq:zh}
	\lim\limits_{t\rightarrow \infty} z(t,\bar{x})=\lim\limits_{t\rightarrow \infty} \frac{1}{t}\sum\limits_{k=1}^{t} \E \left[Q\left(\bar{\Theta}, \bar{\Phi}(k,\bar{\Theta})\right)\right] = h\left(\bar{\Theta}\right)
\end{align}
where $h\left(\bar{\Theta}\right)$ is a bounded and well defined function. Note that
	\begin{widetext}
		\begin{align}\label{eq:EQ}
		\E \left[Q\left(\bar{\Theta}, \bar{\Phi}(k,\bar{\Theta})\right)\right] = 
		\bm{c} 
		\bm{cc} \bar{F}^{-1} & 0 \\ 0 & \bar{f}^{-1}  \mb \E \left\{\bar{\phi}(k, \bar{\Theta}) \left(\bar{y}(k,\bar{\Theta}) - \bar{\theta}^T \bar{\phi}(k, \bar{\Theta})\right)\right\} \\
		\text{\emph{Col}}\left\{ \E\left[\bar{\phi}_1(k,\bar{\Theta}) \bar{\phi}_1^T(k,\bar{\Theta} )\right]  -\bar{F} \right\} \\
		\E \left[ \bar{\Phi}(k, \bar{\Theta})^T M_5^T M_5 \Phi(k) - \bar{f}\right]
		\mb
		\end{align}
	\end{widetext}
and we can show that the limit given in \ref{eq:zh} is well defined for all the three terms on the right hand side. For instance, for the first term we have
	\begin{widetext}
			\begin{align}\label{eq:tmp2}
			\begin{split}
			  \E \left\{\bar{\phi}(k, \bar{\Theta}) \left(\bar{y}(k,\bar{\Theta}) - \bar{\theta}^T \bar{\phi}(k, \bar{\Theta})\right)\right\}  &= \E \left\{\bm{c} \bar{\phi}_1(k,\bar{\Theta}) 
			\\ \phi_R(k) \mb \left(\bar{y}(k,\bar{\Theta}) - \bar{\theta}^T \bar{\phi}(k, \bar{\Theta})\right)\right\}
			\\
			&= \bm{c} \E \left[\bar{\phi}_{1s} (k,\bar{\Theta}) \bar{y}_s(k,\bar{\Theta})\right] +  \bar{\phi}_{1d}(k,\bar{\Theta}) \bar{y}_{d}^T(k,\bar{\Theta}) 
			\\
			\phi_R(k) \bar{y}_d(k,\bar{\Theta}) \mb \\
			&\qquad	  - \bm{c} \bar{\theta_1}^T \E \left[\bar{\phi}_{1s} (k,\bar{\Theta}) \bar{\phi}_{1s}(k,\bar{\Theta})\right]+ \bar{\theta_1}^T \bar{\phi}_{1d}(k,\bar{\Theta}) \bar{\phi}_{1d}^T(k,\bar{\Theta}) + \bar{\theta}_M^T \phi_R(k)\bar{\phi}_{1,d} (k,\bar{\Theta}) \\
			\phi_R(k) \bar{\Phi}_d^T(k,\bar{\Theta})\bar{\theta} \mb
			\end{split}
			\end{align}
	\end{widetext}
where $\bar{\phi}_{1s}(.,.):=M_4\bar{\Phi}_s(.,.)$, $\bar{\phi}_{1d}(.,.):=M_4\bar{\Phi}_d(.,.)$ and $\bar{\theta}_1^T:=\begin{bmatrix}\bar{\theta}_A^T & \bar{\theta}_B^T & \bar{\theta}_C^T\end{bmatrix}$. Similarly, $\bar{y}_d(.,.)$ and $\bar{y}_s(.,.)$ are the values corresponding to $y$ respectively in $\bar{\Phi}_d(.,.)$ and $\bar{\Phi}_s(.,.)$. Note that all the stochastic terms will be stationary when $t\rightarrow\infty$ and all deterministic terms become periodic in steady state. Therefore, all the terms in \eqref{eq:tmp2} when plugged to \eqref{eq:zh} produces well defined limits. Following the same type of analysis, it is easy to show that the second and third terms of \eqref{eq:EQ} generate bounded limits when plugged to \eqref{eq:zh}.

\paragraph*{Assumptions \ref{ass:c4}:} The following analogies between \eqref{eq:z} and \eqref{eq:kv} can be exploited to take the same path as the previous part to show that assumption \ref{ass:c4} holds.
\begin{align*}
z(k,\bar{x})  &\leftrightarrow  k_v(k,\bar{x},\lambda,c) \\
Q(k,\bar{x},\bar{\phi}(k,\bar{x})) &\leftrightarrow \mathscr{K}\left(\bar{x},\bar{\phi}(k,\bar{x}),\rho(\bar{x}),\nu(k,\lambda,c)\right) \\
\mathscr{K}\left(\bar{x},\bar{\phi}(k,\bar{x}),\rho(\bar{x}),\nu(k,\lambda,c)\right) &\leftrightarrow  \mathscr{H}\left(\bar{x},\bar{\phi}(k,\bar{x}),\rho(\bar{x}),\nu(k,\lambda,c),w \right)
\end{align*}



\paragraph*{Assumptions \ref{ass:c5} and \ref{ass:c6}:}
These assumptions are the same as assumption \ref{ass:thm:gamma} in theorem \ref{thm:main}.


\subsection{Convergence Analysis}
Under the regularity conditions mentioned above, the parameter adaptation algorithm \eqref{eq:paa} can be associated with a differential equation that will be derived in this sections.
Suppose the estimate sequence of $\hat{\theta}(k)$ is fixed to a constant value $\hat{\theta}$. Denote $\bar{e}(t,\hat{\theta})$, $\bar{\hat{y}}(t,\hat{\theta})$ and $\bar{\theta}_M(t,\hat{\theta})$ as the (cyclo) stationary processes defined by \eqref{eq:e}, \eqref{eq:yapriori} and \eqref{eq:thetaM}. Note that the stationarity of these processes is admissible only when the closed loop system determined by $\hat{\theta}$ is stable. Suppose $\mathscr{D}_s$ is the set of all values of $\hat{\theta}$ that the stability is attained. The stationary $\tha_D$, by \eqref{eq:integral}, is
\begin{align*}
\bar{\tha}_D(\tha) = \frac{-\alpha}{1-\beta} \hat{D}_B^{-T}(\tha)\tha_M
\end{align*}
where $\hat{D}_B(\tha)$ denotes the value of $\hat{D}_B(k)$ when $\tha(k)=\tha$. Accordingly the control signal associated with $\tha$ is
\begin{align*}
\bar{u}_A(k)= \frac{-\alpha}{1-\beta}\tha_M^T \hat{D}_B^{-1}(\tha)\phi_R(k).
\end{align*}
Therefore, for any fixed $\tha$, the adaptive control algorithm operates in open loop mode and generates a pure feedforward signal. This implies that the closed loop system is stable as long as $\tha_A$ corresponds to an $\hat{A}(\qi)$ polynomial that has all roots strictly inside the unit circle
	\begin{align*}
	\begin{split}
	\mathscr{D}_s:=&\left\{\vphantom{\frac14} \tha:~-\tha_A^T=[\hat{a}_1,\cdots, \hat{a}_{n_A}],\right.\\
	&\qquad \left. {}  1+\hat{a}_1 q +\cdots + \hat{a}_{n_A} q^{{n_A}} =0 \Rightarrow |q|>1 \vphantom{\frac14}\right\}.
	\end{split}
	\end{align*}
This condition is equivalent to assumption \ref{ass:thm:A} in theorem \ref{thm:main}.
The control signal is bounded as long as $\tha_M$ and $\hat{D}_B^{-1}(\tha)\phi_R(k)$ are bounded. The second criterion is equivalent to the condition that $\hat{B}(\qi)$ associated with $\tha_B$ has non-zero magnitude at $\omega_i$'s which is true as long as assumption \ref{ass:thm:B} of theorem \ref{thm:main} holds.
We have
\begin{align*}
\bar{e}(t,\hat{\theta})&=\theta_A \phi_e(t,\hat{\theta}) + \theta_B^T \phi_u(t)+\theta_C^T \phi_{\bar{w}}(t)
\\
&\qquad \qquad \qquad \qquad \qquad   +\bar{\theta}_M^T (t,\hat{\theta}) \phi_R(t)+\bar{w}(t)  \\
\bar{\hat{y}}(t,\hat{\theta})&=\hat{\theta}_A^T \phi_e(t,\hat{\theta}) + \hat{\theta}_B^T \phi_u(t) +\hat{\theta}_C^T \phi_{\epsilon}(t,\hat{\theta}) + \hat{\theta}_M^T {\phi}_R(t,\hat{\theta})
\end{align*}
In the first expression, we have used $w_t(t,\hat{\theta})=0$ since the term $\left(z-1\right)\left[\theta(k)\right]$ in  lemma \ref{lemma:swapping} is zero once $\hat{\theta}(k)$ is frozen. 
The stationary estimation error defined in \eqref{eq:eapriori} is
		\begin{align*}
			&\bar{\epsilon}(t,\tha) = \bar{e}(t,\hat{\theta}) - \bar{\hat{y}}(t,\hat{\theta})\\
			&=\left({\theta}_A^T-\hat{\theta}_A^T\right) \phi_e(t,\hat{\theta}) + \left({\theta}_B^T-\hat{\theta}_B^T\right) \phi_u(t) \\
			&~~~+ \left({\theta}_C^T-\hat{\theta}_C^T\right) \phi_{\epsilon}(t,\hat{\theta}) - \theta_C \phi_{\epsilon}(t,\hat{\theta})+\theta_C^T \phi_{\bar{w}}(t) \\
			&~~~+\bar{\theta}_M^T (t,\hat{\theta}) \phi_R(t)-\hat{\theta}_M^T {\phi}_R(t,\hat{\theta}) + \bar{w}(t)\\
		\end{align*}

By using $\theta_C^T \phi_{\bar{w}}(t)+ \bar{w}(t) = C(\qi)\bar{w}(t)$ and ${\theta}_C^T \phi_{\epsilon}(t,\hat{\theta})+ \bar{\epsilon}(t,\tha)  = C(\qi)\bar{\epsilon}(t,\tha)$
we have
		\begin{align}\label{eq:eps1}
		\begin{split}
			\bar{\epsilon}(t,\tha) &= \frac{1}{C(\qi)}\left[\left({\theta}_A^T-\hat{\theta}_A^T\right) \phi_e(t,\hat{\theta}) + \left({\theta}_B^T-\hat{\theta}_B^T\right) \phi_u(t)\right.\\
			&\left. +  
			 \left({\theta}_C^T-\hat{\theta}_C^T\right) \phi_{\epsilon}(t,\hat{\theta}) +\bar{\theta}_M^T (t,\hat{\theta}) \phi_R(t)-\hat{\theta}_M^T {\phi}_R(t,\hat{\theta})\right] + \bar{w}(t)
			\\
			&=\frac{1}{C(\qi)} \begin{bmatrix} \phi_e(t,\hat{\theta})\\ \phi_u(t)\\ \phi_{\epsilon}(t,\hat{\theta}) \\\phi_R(t) \end{bmatrix}^T
			\begin{bmatrix}
			{\theta}_A-\hat{\theta}_A \\ {\theta}_B-\hat{\theta}_B \\ {\theta}_C-\hat{\theta}_C \\ \bar{\theta}_M(t,\tha) -  \hat{\theta}_M
			\end{bmatrix}+ \bar{w}(t)
		\end{split}
		\end{align}
	
%The scaled rotation matrix $\Delta(\tha)$ satisfies $\hat{\phi}_R(t)=\Delta(\tha){\phi}_R(t,\tha)$.
The stationary process $\bar{\theta}_M(t,\tha)$ can be derived from \eqref{eq:thetaM} and \eqref{eq:integral}
	\begin{align*}\notag
		\theta_M(k+1) &= {D}_B^{T}\tha_D(k+1)+\theta_R \\\notag
		&=\beta {D}_B^{T}\tha_D(k) - \alpha {D}_B^{T}\hat{D}_B^{-T}(k) \tha_M(k)  + \theta_R\\\notag
		%&=\beta \left({D}_B^{T}(k)\tha_D(k) + \theta_R\right)  - \alpha {D}_B^{T}\hat{D}_B^{-T}(k) \tha_M(k)+\left(1-\beta\right) \theta_R \\\notag
		&=\beta \theta_M(k)  - \alpha \Delta^T(\tha) \tha_M(k)+\left(1-\beta\right) \theta_R
	\end{align*}
where $\Delta(\tha)$ is the stationary matrix for $\Delta(k)$ and
	\begin{align*}
		\Delta(k):&= \hat{D}_B^{-1}(k)D_B\\
%		&=\begin{bmatrix}
%		\hat{D}_{B1}^{-1}(k) & 0 & \cdots & 0\\
%		0 & \hat{D}_{B2}^{-1}(k) & \cdots & 0\\
%		\vdots & \vdots &\ddots & \vdots\\
%		0 & 0 & \cdots & \hat{D}_{Bn}^{-1}(k)
%		\end{bmatrix}
%		\begin{bmatrix}
%		{D}_{B1} & 0 & \cdots & 0\\
%		0 & {D}_{B2} & \cdots & 0\\
%		\vdots & \vdots &\ddots & \vdots\\
%		0 & 0 & \cdots & {D}_{Bn}
%		\end{bmatrix}\\
		&=\begin{bmatrix}
		\hat{D}_{B1}^{-1}(k) {D}_{B1} & 0 & \cdots & 0\\
		0 & \hat{D}_{B2}^{-1}(k) {D}_{B2} & \cdots & 0\\
		\vdots & \vdots &\ddots & \vdots\\
		0 & 0 & \cdots & \hat{D}_{Bn}^{-1}(k) {D}_{Bn}
	\end{bmatrix}
	\end{align*}
\begin{align*}
\hat{D}_{Bi}^{-1}(k) {D}_{Bi} &= \left(\frac{1}{\hat{m}_{Bi}} R\left(-\hat{\delta}_{Bi}(k)\right)\right)\left({{m}_{Bi}} R\left(\delta_{Bi}\right)\right)\\
&=\frac{m_{Bi}}{\hat{m}_{Bi}(k)} R(\delta_{Bi}-\hat{\delta}_{Bi}(k))
\end{align*}
Therefore,
\begin{align*}
\bar{\theta}_M(t,\tha) &= \beta \bar{\theta}_M(t,\tha) - \alpha \Delta^T(\tha) \tha_M+\left(1-\beta\right) \theta_R\\
&=\theta_R-\frac{\alpha}{1-\beta}\Delta^T(\tha)\tha_M.
\end{align*}
%Let $\Delta(\tha)$ be a weighted rotation matrix that maps $\hat{\phi}_R(t,\tha)$ to $\phi_R(t)$
%\begin{align*}
%\phi_R(t)=\Delta(\tha)\hat{\phi}_R(t,\tha).
%\end{align*}
Using this definition and the expression for $\bar{\theta}_M$ we have
\begin{align*}
	&\bar{\theta}_M^T (t,\hat{\theta}) \phi_R(t)-\hat{\theta}_M^T {\phi}_R(t) 
	\\ 
	&\qquad \qquad =
	{\phi}_R^T(t)
	\left(I+\frac{\alpha}{1-\beta}\Delta^T(\tha)\right) 
	\left[\theta_M^*-\tha_M\right]
\end{align*}
where
\begin{align}\label{eq:thetaMStar}
\theta_M^* = \left(I+\frac{\alpha}{1-\beta}\Delta(\tha)\right)^{-T}\theta_R.
\end{align}
The expression $I+\frac{\alpha}{1-\beta}\Delta(\tha)$ has singularity point at 
	\begin{align}\label{eq:singularity}
	\begin{split}
		\hat{\delta}_{B_i}&=\delta_{B_i}-\pi\\
		\hat{m}_{B_i}&=\frac{\alpha}{1-\beta}m_{B_i}.
	\end{split}
	\end{align}
By choosing appropriate $\alpha$ and $\beta$ and limiting $\hat{m}_{B_i}$ from above, the singularity point can be avoided. This condition is guaranteed by assumption \ref{ass:thm:B} in theorem \ref{thm:main}. However, as we will see in the sequel, the algorithm avoids such a large phase difference $\delta_{B_i}-\hat{\delta}_{B_i}=\pi$ with probability one even no upper bound is applied to $\hat{m}_{B_i}$.
 
Returning to \eqref{eq:eps1}, we have
	\begin{align}\label{eq:eps2}
	\begin{split}
		& \bar{\epsilon}(t,\tha) =\frac{1}{C(\qi)} 
		\left[\begin{array}{c} \phi_e(t,\hat{\theta})\\ \phi_u(t)\\ \phi_{\epsilon}(t,\hat{\theta}) \\ \hdashline {\phi}_R(t) \end{array}\right]^T
		\times \\
		& \qquad\qquad \left[\begin{array}{c:c} I & 0 \\ \hdashline 0 & I+\frac{\alpha}{1-\beta}\Delta^T(\tha) \end{array}\right]
		\left[\begin{array}{c} {\theta}_A-\hat{\theta}_A \\ {\theta}_B-\hat{\theta}_B \\ {\theta}_C-\hat{\theta}_C \\ \hdashline \theta_M^* -  \hat{\theta}_M \end{array}\right]
	\end{split}
	\end{align}
When $\Delta$ is bounded, by choosing $\beta$ close enough to 1 and $\alpha \gg 1-\beta$ the inverse term is not subjected to numerical issues and $\theta_M^* \ll \theta_R$.

Introduce 

	\begin{widetext}
			\begin{subequations}\label{eq:G-all}
				\begin{align}
				\label{eq:Gtilde}
				\tilde{G}(\tha) 
				: &=
				\frac{1}{t}\sum\limits_{k=1}^{t} \left(
				\left[\begin{array}{c} \phi_e(k,\hat{\theta})\\ \phi_u(k)\\ \phi_{\epsilon}(k,\hat{\theta}) \\{\phi}_R(k) \end{array}\right]
				\left[\begin{array}{c:c}    \frac{1}{C(\qi)} & 0 \\ \hdashline  0 & \frac{1+H(q^{-1};\tha)}{C(\qi)}  \end{array}\right]
				\left[\begin{array}{c} \phi_e(k,\hat{\theta})\\ \phi_u(k)\\ \phi_{\epsilon}(k,\hat{\theta}) \\ {\phi}_R(k) \end{array}\right]^T\right)
				\\
				\label{eq:G}
				G(\tha):&= \frac{1}{t}\sum\limits_{k=1}^{t} 
				\left[\begin{array}{c} \phi_e(k,\hat{\theta})\\ \phi_u(k)\\ \phi_{\epsilon}(k,\tha)\end{array} \right]
				\\
				\label{eq:gsmall}
				g(\tha):&=\frac{1}{t}\sum\limits_{k=1}^{t} {\phi}_R^T(k){\phi}_R(k)
				\end{align}
			\end{subequations}
	\end{widetext}
%
and decompose $\phi_e(k)$ to a stochastic and deterministic part as $\phi_e(k)=\phi_{ed}(k)+\phi_{es}(k)$. The fact that all stochastic processes are zero mean along with \eqref{eq:sumToExpect} imply
%
	\begin{widetext}
			\begin{align}
			\tilde{G}(\tha)& \rightarrow \tilde{G}_s(\tha)+\tilde{G}_d(\tha) \qquad \text{w.p. 1 as }t\rightarrow \infty
			\\
			\tilde{G}_s(\tha)&:=\E \left(
			\begin{bmatrix} \phi_{es}(k,\hat{\theta})\\ 0\\ \phi_{\epsilon}(k,\hat{\theta}) \\0 \end{bmatrix}
			\frac{1}{C(\qi)} 
			\begin{bmatrix} \phi_{es}(k,\hat{\theta})\\ 0\\ \phi_{\epsilon}(k,\hat{\theta}) \\ 0 \end{bmatrix}^T\right)
			\\
			\tilde{G}_d(\tha)&:=\frac{1}{t}\sum\limits_{k=1}^{t} \left(
			\begin{bmatrix} \phi_{ed}(k,\hat{\theta})\\ \phi_u(k)\\ 0 \\ \hdashline  {\phi}_R(k) \end{bmatrix}
			\left[\begin{array}{c:c}    \frac{1}{C(\qi)} & 0 \\ \hdashline  0 & \frac{1+H(q^{-1};\tha)}{C(\qi)}  \end{array}\right]
			\begin{bmatrix} \phi_{ed}(k,\hat{\theta})\\ \phi_u(k)\\ 0 \\ \hdashline {\phi}_R(k) \end{bmatrix}^T\right)
			\end{align}
	\end{widetext}
	
Here, $H(\qi, \tha)$ is a stable and causal transfer function, e.g. an FIR LTI system, that at $\omega_i$'s has magnitude and phase responses equal to the corresponding magnitudes and phases in $ \frac{\alpha}{1-\beta}\Delta^T(\tha)$. It is trivial that such an LTI transfer function can be found for any $\Delta^T(\tha)$ by considering at most $2n$ coefficients.

Under the regularity conditions and conditions on the stochastic processes $\bar{w}(k)$ and $u(k)$ that were mentioned above the parameter adaptation algorithm in \eqref{eq:paa} can be associated with the differential equation \cite{ljung1977analysis}
\begin{subequations}\label{eq:ode}
\begin{align}\label{eq:ode-theta}
\frac{d}{dt}\hat{\theta}(t)&=\bm{cc} F^{-1}(t) & 0 \\ 0 & f^{-1}(t)I \mb 
\tilde{G}(\tha(t))
%\left[\begin{array}{c:c} I & 0 \\ \hdashline 0 & \frac{\alpha}{1-\beta}I+\Delta^T(\tha) \end{array}\right]
\begin{bmatrix} {\theta}_A-\hat{\theta}_A \\ {\theta}_B-\hat{\theta}_B \\ {\theta}_C-\hat{\theta}_C \\ \theta_M^* -  \hat{\theta}_M \end{bmatrix}
\\ 
\label{eq:ode-F}
\frac{d}{dt} F(t)&=G(\tha(t))-F(t)
\\
\label{eq:ode-f}
\frac{d}{dt} f(t)&=g(\tha(t))-f(t).
\end{align}
\end{subequations}
Moreover, the convergence point(s) of parameter adaptation algorithm \eqref{eq:paa} can be related to the set of stationary points, say $\mathscr{D}_c$, of the differential equations \eqref{eq:ode} through corollary 1 in \cite{ljung1977analysis}. The following conditions, that are already shown to be satisfied partially, are required to use the corollary results
\begin{itemize}
	\item 
	Regularity conditions mentioned above should be satisfied.
	\item
	$\tha(k) \in \mathscr{D}_s$ infinitely often with probability one.
	\item
	$\|{\phi}(k)\|$ is bounded infinitely often whenever $\tha(k)$ belongs to $\mathscr{D}_s$
	\item
	There is a Lyapunov function $V\left(\tha(t), F(t), f(t)\right)$ such that 
	\begin{align*}
	\frac{d}{dt} V\left(\tha(t), F(t), f(t)\right)&\le 0 \quad \text{for  }\tha(t)\in \mathscr{D}_s,~F(t)>0,~f(t)>0\\
	\frac{d}{dt} V\left(\tha(t), F(t), f(t)\right)&= 0 \quad \text{for  }\tha(t)\in \mathscr{D}_c
	\end{align*}
\end{itemize}
We have already shown that the first condition is satisfied  when a projection scheme is considered. The third condition can be satisfied by restricting $\tha_B(k)$ to
\begin{align*}
\mathscr{D}_B:=
\left\{\vphantom{\frac12}  \tha_B : |b_1^i e^{-j\omega_m} + \cdots + b_{n_A}^i  e^{-jn_A \omega_m}|>0  \right. \\
\left. \forall i \in \{1,\ldots, n_i\} \text{  and  } \forall m \in \{1,\ldots,n\} \vphantom{\frac12}  \right\}.
\end{align*}
This means that the magnitude of $\hat{B}(\qi;k)$ at excitation frequencies should be bounded  from below by a small positive value. This is equivalent to assumption \ref{ass:thm:B} in theorem \ref{thm:main}. In case $\tha_B(k)$ does not belong to $\mathscr{D}_B$, the parameters can be projected to $\mathscr{D}_B$ by scaling $\tha_B(k)$.
%This results in boundness of ${\phi}_R(k)$ and accordingly $\hat{\phi}(k)$. 
An implication of this restriction is that $\Delta(\tha(k))$ is also always bounded. 
%This is a useful fact for the last condition because the term $\frac{\alpha}{1-\beta}I+\Delta^T(\tha)$ will be positive definite by choosing $\beta$ close (from left) enough to 1. 

Analogous to \cite{ljung1977positive} an admissible Lyapunov function can be defined when $\tilde{G}(\tha)+\tilde{G}^T(\tha)$ is positive definite. This is possible when both $\frac{1}{C(\qi)}$ and $\frac{H(\qi,\tha)}{C(\qi)}$ are strictly positive real. The second condition can be relaxed further since the response of $H(\qi; \tha)$ is only important at $\omega_i$'s. Therefore, $\tilde{G}(\tha)+\tilde{G}^T(\tha)$ is positive definite if
\begin{enumerate}
	\item $\phi_u$ is persistently exciting of order $2n$.
	\item $\frac{1}{C(\qi)}$ is strictly positive real (SPR).
	\item Absolute phase of $\frac{H(e^{-j\omega_i}; \tha)}{C(e^{-j \omega_i})}$ is less than $90$ degrees.
\end{enumerate}
%The third condition can be justified by comparing \eqref{eq:Gtilde} with
%\begin{align*}
%\left[\begin{array}{c} \phi_1\\ \phi_2\end{array}\right]
%\left[\begin{array}{cc}    \frac{1}{C} & 0 \\   0 & \frac{1+H}{C}  \end{array}\right]
%\left[\begin{array}{c} \phi_1\\ \phi_2\end{array}\right]^T 
%&= 
%\left[\begin{array}{c} \phi_1\\ \phi_2\end{array}\right]
%\frac{1}{C}
%\left[\begin{array}{c} \phi_1\\ \phi_2\end{array}\right]^T
%+
%\left[\begin{array}{cc}    0 & 0 \\   0 & \phi_2 \frac{H}{C}\phi_2^T  \end{array}\right].
%\end{align*}
%If $1/C(\qi)$ is strictly positive real, the first term on the left will make a positive definite matrix when it is summed with its transpose. Similarly, when $H(\qi)/C(\qi)$ is SPR, summation of the second term with its transpose results in a positive semi-definite matrix. This implies that the summation of the two transfer functions results in a positive definite matrix when condition 2 and 3 hold.
%
Note that these conditions are equivalent to assumptions \ref{ass:thm:u},\ref{ass:thm:C} and \ref{ass:thm:H} of theorem \ref{thm:main} respectively.



\begin{proof}[Theorem \ref{thm:main}]
Theorem 2 in \cite{ljung1977analysis} implies that the convergence point(s) of the parameter adaptation algorithm \eqref{eq:paa} are among the stable  stationary points of \eqref{eq:ode}. For an SPR $1/C(\qi)$, the cross covariance matrix 
\begin{align*}
\frac{1}{t}\sum\limits_{k=1}^{t} \left(
\left[\begin{array}{c} \phi_e(k,\hat{\theta})\\ \phi_u(k)\\ \phi_{\epsilon}(k,\hat{\theta}) \\{\phi}_R(k) \end{array}\right]
\frac{1}{C(\qi)}
\left[\begin{array}{c} \phi_e(k,\hat{\theta})\\ \phi_u(k)\\ \phi_{\epsilon}(k,\hat{\theta}) \\ {\phi}_R(k) \end{array}\right]^T\right)
\end{align*}
added to its transpose makes a positive definite matrix. Therefore, from \eqref{eq:eps2}, the only stationary point of \eqref{eq:ode-theta} is given by
\begin{align*}
\left[\begin{array}{c:c} I & 0 \\ \hdashline 0 & I+\frac{\alpha}{1-\beta}\Delta^T(\tha) \end{array}\right]
\left[\begin{array}{c} {\theta}_A-\hat{\theta}_A \\ {\theta}_B-\hat{\theta}_B \\ {\theta}_C-\hat{\theta}_C \\ \hdashline \theta_M^* -  \hat{\theta}_M \end{array}\right]\
=0.
\end{align*}
The left matrix singularity points are described in \eqref{eq:singularity}. It is trivial that the parameter $\hat{\theta}_B$ corresponding to such a singularity point does not fall in the null space of the left matrix. 
Hence, the only stationary point of \eqref{eq:ode} is
	\begin{align*}
		\theta^*
		=
		\left[\begin{array}{c} \hat{\theta}_A \\ \hat{\theta}_B \\ \hat{\theta}_C \\  \hat{\theta}_M \end{array}\right]
		=
		\left[\begin{array}{c} {\theta}_A \\ {\theta}_B\\ {\theta}_C\\ \frac{1-\beta}{1-\beta+\alpha} \theta_R \end{array}\right] 
	\end{align*} 
where the last term comes from \eqref{eq:thetaMStar} when $\tha_B=\theta_B$.
Moreover, it can be shown that this is a locally stable stationary point. 
Suppose $\B(\theta_B,\rho(\theta_B))$ be a neighborhood of $\theta_B$ in which $|\delta_{B_i}-\hat{\delta}_{B_i}|<90$. The quadratic function
\begin{align*}
V(\tha):=\tha^T\left(\tilde{G}(\tha)+\tilde{G}^T(\tha)\right)\tha.
\end{align*}
is positive definite and has negative definite Lie derivative along \eqref{eq:ode} trajectories as long as $\tha \in \B(\theta^*,\rho(\theta_B))$. 
This is because  $\|\theta_B-\tha_B\|\le \|\theta^*-\tha\|$ implies that starting the trajectory from $\tha(0) \in \B(\theta^*,\rho(\theta_B))$, the estimated $\tha_B$ always stays in a neighborhood with a smaller radius around $\theta_B$. Therefore, decreasing $\|\theta^*-\tha\|$ results in keeping $\tha_B$ in $\B(\theta^*,\rho(\tha_B))$ which itself implies more reduction in  $\|\theta^*-\tha\|$.
Accordingly, $V(\tha)$ is a Lyapunov function for \eqref{eq:ode} and the equilibrium state $\theta^*$ is stable in the sense of Lyapunov.






%
%
%\section{proof junks}
%The ``free response'' of \eqref{eq:M} is governed by the time varying matrix $( I - \alpha_k  \Delta_B(k))$. A (conservative) criterion for the convergence of this term to zero can be found based on the maximum singular value of this matrix
%\begin{align*}
%\frac{\left\|\left( I - \alpha_k  \Delta_B\left(k\right)\right)\theta_M(k)\right\|}{\left\|\theta_M(k)\right\|} \le \sigma_{\max}\left(I - \alpha_k  \Delta_B\left(k\right)\right) \le 1
%\end{align*}
%where $\sigma_{\max}(.)$ denotes the maximum singular value. Since the singular values are non-negative, we have
%\begin{align}\nt
%1 &\ge \sigma_{\max}^2\left(I - \alpha_k  \Delta_B\left(k\right)\right)  \\ \nt
%&=\lambda_{\max}\left[\left(I - \alpha_k  \Delta_B\left(k\right)\right)\left(I - \alpha_k  \Delta_B\left(k\right)\right)^T\right] \\\nt
%&=\lambda_{\max}\left[I - \alpha_k \left( \Delta_B \left(k\right) +\Delta_B^T\left(k\right)\right)+ \alpha_k^2  \Delta_B \left(k\right) \Delta_B^T\left(k\right)\right] \\ \label{eq:lambdamax}
%&=1+\lambda_{\max}\left[ - \alpha_k \left( \Delta_B \left(k\right) +\Delta_B^T\left(k\right)\right)+ \alpha_k^2  \Delta_B \left(k\right) \Delta_B^T\left(k\right)\right]
%\end{align}
%Using the following two relations
%\begin{align*}
%\hat{D}_{Bi}^{-1}(k) {D}_{Bi}+\left(\hat{D}_{Bi}^{-1}(k) {D}_{Bi}\right)^T &= \frac{m_{Bi}}{\hat{m}_{Bi}(k)}\left[ R(\delta_{Bi}-\hat{\delta}_{Bi}(k))+R(\hat{\delta}_{Bi}(k)-\delta_{Bi})\right]\\
%&=2\frac{m_{Bi}}{\hat{m}_{Bi}(k)}\cos(\hat{\delta}_{Bi}(k)-\delta_{Bi}) I\\
%\hat{D}_{Bi}^{-1}(k) {D}_{Bi}\left(\hat{D}_{Bi}^{-1}(k) {D}_{Bi}\right)^T &=\left(\frac{m_{Bi}}{\hat{m}_{Bi}(k)}\right)^2\left[ R(\delta_{Bi}-\hat{\delta}_{Bi}(k)) R(\hat{\delta}_{Bi}(k)-\delta_{Bi})\right]\\
%&=\left(\frac{m_{Bi}}{\hat{m}_{Bi}(k)}\right)^2 {I}
%\end{align*}
%implies that \eqref{eq:lambdamax} is equivalent to
%\begin{gather}\nt
%0\ge \max\limits_{i}\left(\lambda\left[ - 2\alpha_k \frac{m_{Bi}}{\hat{m}_{Bi}(k)}\cos(\hat{\delta}_{Bi}(k)-\delta_{Bi}) I+ \alpha_k^2  \left(\frac{m_{Bi}}{\hat{m}_{Bi}(k)}\right)^2 {I}\right]\right)\\\nt
%=\alpha_k \frac{m_{Bi}}{\hat{m}_{Bi}(k)}\max\limits_{i}\left( - 2\cos(\hat{\delta}_{Bi}(k)-\delta_{Bi}) + \alpha_k  \frac{m_{Bi}}{\hat{m}_{Bi}(k)}\right)\Leftrightarrow\\ \label{eq:alp}
%0\le \alpha_k  \frac{m_{Bi}}{2\hat{m}_{Bi}(k)}\le  \cos(\hat{\delta}_{Bi}(k)-\delta_{Bi})  \quad \text{for} \quad 1\le i \le n.
%\end{gather}
%This inequality implies that when the phase mismatch between the identified and actual transfer function of $B(\qi)$ is less than 90 degrees and $\alpha_k$ is chosen small enough such that 
%\begin{align*}
%0\le \alpha_k \le \min\limits_{i} \frac{\cos(\hat{\delta}_{Bi}(k)-\delta_{Bi})  }{\frac{m_{Bi}}{2\hat{m}_{Bi}(k)}}
%\end{align*}
%the free response in \eqref{eq:M} converges to zero.
%
\end{proof}
\begin{proof}[Theorem \ref{lemma:usingCbar}]
	The proof of theorem \ref{lemma:usingCbar} is similar to the proof of theorem \ref{thm:main} up to equation \eqref{eq:eps2}. 
	Starting from \eqref{eq:G-all}, one needs to substitute all instances of $C(\qi)$ by $C(\qi)/\bar{C}(\qi)$ to show the results.
\end{proof}

\begin{proof}[Theorem \ref{thm:main2}]
	The proof is based on to the proof of theorem \ref{thm:main}.	
	When there is no prior knowledge regarding $B(\qi)$ in hand, it may not be possible to set the initial conditions of \eqref{eq:paa} and accordingly \eqref{eq:ode} to guarantee SPR condition on $H(\qi; \tha)/C(\qi)$ term. However, the region of attraction for differential equation \eqref{eq:ode} can be enlarged in practice by increasing the excitation energy. Consider the upper states of \eqref{eq:ode-theta} 
	
	\begin{widetext}
		\begin{align}\label{eq:paa_ode_upperpart}
		\begin{split}
		\frac{d}{dt}\begin{bmatrix} \hat{\theta}_A \\ \hat{\theta}_B \\ \hat{\theta}_C \end{bmatrix}&=F^{-1}(t)
		%
		\frac{1}{t}
		%
		\sum\limits_{k=1}^{t} \left(
		\left[\begin{array}{c} \phi_e(k,\hat{\theta})\\ \phi_u(k)\\ \phi_{\epsilon}(k,\hat{\theta})  \end{array}\right]
		\frac{1}{C(\qi)} 
		\left[\begin{array}{c} \phi_e(k,\hat{\theta})\\ \phi_u(k)\\ \phi_{\epsilon}(k,\hat{\theta})  \end{array}\right]^T\right)
		\begin{bmatrix} {\theta}_A-\hat{\theta}_A \\ {\theta}_B-\hat{\theta}_B \\ {\theta}_C-\hat{\theta}_C  \end{bmatrix}
		\\
		&\qquad \qquad\qquad\qquad\qquad\qquad\qquad 
		+F^{-1}(t)\frac{1}{t}
		\sum\limits_{k=1}^{t} 
		\left[\begin{array}{c} \phi_e(k,\hat{\theta})\frac{1+H(\qi; \tha)}{C(\qi)} \phi_R^T(k)\\ 0\\ 0  \end{array}\right]
		\theta_M^* -  \hat{\theta}_M
		\end{split}
		\end{align}
	\end{widetext}
	when $1/C(\qi)$ is SPR, the first term on the right attracts the states to $\begin{bmatrix}\theta_A^T & \theta_B^T & \theta_C^T\end{bmatrix}^T$. However, the second term might be repulsive when $H(\qi; \tha)/C(\qi)$ is not SPR. 
	 In \eqref{eq:paa_ode_upperpart}, the second term on the right hand side is 
	 bounded when assumption \ref{ass:thm2:thetabounded} in theorem \ref{thm:main2} holds true. As a result, by increasing $\alpha_{dc}$ the attraction of the first term increases which can lead to bringing $\tha_B$ into $\mathscr{D}_B$ when $\alpha_{dc}$ is chosen large enough.  
	 This means that by choosing enough excitation in such a case, the convergence rate of the first term can be increased such that the first term brings $\tha_B$ into a vicinity of $\theta_B$ in which the second term is also attractive.
\end{proof}

==> excitation_signal.tex <==
% =======================================================================================
\section{Exogenous Excitation Signal}\label{sec:excitationSignal}
Assumption \ref{ass:thm:u} requires a ``frequency rich'' excitation signal $u(k)$. 
The standard solution in practice is usually provided by the use of \emph{pseudo--random binary sequences} that have enough persistence of excitation for identification of any number of parameters \cite{bitmead1984persistence}. 
As stated above, the domain of attraction can be enlarged by increasing the power of this excitation signal. 
However, exciting the system with a large exogenous signal may not be practical or desirable in many applications.

The (pseudo--) random excitations are usually beneficial when the identification should be performed in a wide frequency range due to their flat power spectral density.  
In our problem, based on assumption \ref{ass:thm:H} (or \ref{ass:thm:H2}), the system dynamics is important only around the compensation frequencies ($\omega_i$'s).
%Therefore, rather than a pseudo--random excitation, we propose using a special excitation that contains narrow--band contents. As a result, 
%We propose a method that requires less computation and it is more effective for our problem because we need to identify the system dynamics only around the narrow band disturbances. 
%The fact that the adaptive algorithms can operate with extremely weak excitation signals is a very much appreciated quality in practical situations.
We propose shaping the excitation power spectral density such that all power is focused around the narrow--band disturbances. 
This approach has two advantages: 
(1) the excitation adverse effect can be considerably decreased 
by removing the frequency contents that does not provide any ``useful'' information to the adaptive algorithm,
(2) the number of parameters in $\tha_A$ and $\tha_B$ can be decreased because they only need to capture the system dynamics around $\omega_i$'s.

We propose using sinusoidal excitations that are distributed symmetrically around compensation frequencies ($\omega_i$)
%The excitation signal superposes sinusoidal terms symmetric around compensation frequencies
	\begin{align}\label{eq:u1}
	u(k)=\frac{\alpha^u(k)}{2} \sum\limits_{i=1}^{n} \sin\left((\omega_i + \delta_u)kT\right) + \sin\left((\omega_i - \delta_u)kT\right) .
	\end{align}
%which implies that the whole excitation energy is focused sharply around where identification should be performed. 
Here, $\delta_u$ is a small frequency shift such as a few percent of the smallest $\omega_i$, and $\alpha^u(k)$ is a fixed or variable positive gain that should be defined based on the noise level, desired convergence rate and unwanted transient error. 
%An adaptive version of this gain is discussed in section \ref{sec:exciationGain}.

Although this excitation signal contains many sinusoidals, it can be constructed with negligible computation when combined with
the proposed adaptive feedforward controller. This is because 
the expression in \eqref{eq:u1} can be effectively evaluated by taking advantage of the regressor $\phi(k)$ due to the fact that
	\begin{align}\label{eq:excitation_simplified}
	\begin{split}
		u(k)%&=\frac{\alpha^u(k)}{2} \sum\limits_{i=1}^{n} \sin\left((\omega_i + \delta_u)kT\right) + \sin\left((\omega_i - \delta_u)kT\right) \\
		%&=\frac{\alpha^u(k)}{2}\sum\limits_{i=1}^{n} \sin(\omega_i kT) \cos(\delta_u kT) + \cos(\omega_i kT) \sin(\delta_u kT) \\
		%&\qquad \qquad \qquad + \sin(\omega_i kT) \cos(\delta_u kT) - \cos(\omega_i kT) \sin(\delta_u kT)\\
		&={\alpha^u(k)}\cos(\delta_u kT)\sum\limits_{i=1}^{n} \sin(\omega_i kT)\\
		&={\alpha^u(k)}\cos(\delta_u kT)\sum\limits_{i=1}^{n} \phi_{2i-1}(k).
	\end{split}
	\end{align}
%Note that all trigonometric functions in front of the sum operator have been already evaluated for $\phi(k)$. 
Thus, even though the excitation signal consists of $n+1$ trigonometric functions, only one function evaluation is needed and the rest is in hand once the regressor $\phi(k)$ is calculated.
Note that this signal is persistently exciting of order $2n$. In case it does not satisfy assumption \ref{ass:thm:u}, similar terms with different $\delta_u$'s can be added.




%As a rule of thumb, the smoothing factor in exponential smoothing is usually chosen from $\left[0.001, 0.01\right]$. The initial guess for the DC gain depends on the actuator saturation limit.

%\subsection{Spectrum Partitioning}\label{sec:partitioning}
%Let $\Omega$ be the set of all compensation frequencies
%\begin{align*}
%\Omega:=\{\omega_i | 1\le i \le n\}.
%\end{align*}
%As mentioned earlier, there are two main constraints that prevent us from compensating all of these frequencies by a single controller module when $n$ is large, $\omega_i$'s are spread and the system frequency response is complicated: 
%(1) the embedded processor may not have enough computation power to perform one step update of all parameters in one sampling interval 
%(2) a high order model (i.e. large $n_A$) may be needed to capture the dynamics of system at a broad frequency range.
%
%Our objective is to divide $\Omega$ to a collection of subsets, run the adaptive controller on these regions subsequently and superpose the feed--forward control signal learned in each region in order to synthesize a general control signal that attenuates all narrow--band disturbances at frequencies contained in $\Omega$.  More explicitly, we look for 
%\begin{itemize}
%\item a collection, say $C:\{\Omega_j|1\le j \le m\}$, of mutually disjoint non--empty sets whose union is $\Omega$.
% \item each subset contains consecutive elements
% \item a low order model can be fit to the actual system dynamics in each region
% \item the number of subsets, $m$, is kept as small as possible
% \item the running time needed to perform the algorithm does not exceed the sampling time of the system, which means that, the size of subsets should be bounded by a particular number that depends on the available computational power.
%\end{itemize}
%An admissible partition depends on the complexity of system dynamics and the controller processing unit. We propose a heuristic algorithm inspired by divisive hierarchical clustering \cite{rokach2005clustering}  in conjunction with a monitoring mechanism to perform the partitioning in an online fashion. 
%Let 
%$$C(t):=\{\Omega_j(t)|1\le j \le m(t)\}$$
%be the collection at iteration $t$ and assume that subsets $\Omega_j(t)$ are ordered such that the largest frequency in $\Omega_{j1}(t)$ is strictly less than the smallest frequency in $\Omega_{j2}(t)$ if and only if $j1<j2$. We use $\Omega_{j1}(t)<\Omega_{j2}(t)$ notation for this type of set ordering.
%The collection is initialized with only one cluster 
%$$\Omega_0(0)=\Omega.$$
%Let $M_i(k):=\|\tha_{M,2i-1}(k)+j\tha_{M,2i}(k)\|$, where $\tha_{M,i}(k)$ denotes the i-th element of $\tha_M(k)$ and $j$ is the imaginary unit only in this particular expression. Indeed, $M_i(k)$ is the magnitude of residue corresponding to $\omega_i$ at time step $k$. 
%At iteration $t$ the adaptive algorithm is applied on region $\Omega_c(t)$ for $N$ steps and the $\mathcal{L}_\infty$ norm of $M^T(k):=[M_1(k),\cdots,M_n(k)]$ is monitored. Two cases are considered:
%\begin{itemize}
%	\item[I.]
%	$\|M(k)\|_\infty$ is increased for a particular number of consequent steps, say $n_{fail}$, before reaching step $N$: it indicates divergence of residues and the adaptive algorithm will be terminated. In this case of early termination, the current region $\Omega_c(t)$ will be divided to two regions $\Omega^1<\Omega^2$. $\Omega^1$ which is the first half of $\Omega_c(t)$ will be the region under verification in the next iteration and $\Omega^2$ will be merged to the next region. That is
%		\begin{align}\label{eq:direct_omegaSplit}
%		\begin{split}
%		\Omega_{c+1}(t)&\gets \Omega_{c+1}(t)\cup \Omega^2\\
%		C(t+1)&\gets \left(C(t) - \{\Omega_c(t)\}\right) \cup  \{\Omega^1\}.
%		\end{split}
%		\end{align}
%	Note that in this case $c$ is not updated. Therefore, $\Omega_c(t+1)=\Omega^1$.
%	
%	\item[II.]
%	Otherwise: in this case no divergence is indicated. Therefore, $\Omega_c(t)$ is an admissible region and we need to check the next region in the next iteration 
%	$$c\leftarrow c+1.$$
%\end{itemize}
%The pseudo--code for this algorithm is given in Algorithm~\ref{alg:specpart}. $\texttt{AdaptiveControl}(\Omega_c(t))$ refers to applying the proposed adaptive control algorithm to region $\Omega_c(t)$. Function \texttt{Divide(.)} in the algorithm splits $\Omega_c(t)$ to $\Omega^1$ and $\Omega^2$ such that $\Omega^1\ne \emptyset$, $\Omega^2\ne \emptyset$, $\Omega^1< \Omega^2$, $\Omega^1 \cap \Omega^2 = \emptyset$ and $\Omega^1 \cup \Omega^2 =\Omega_c(t)$. A natural solution can be obtained by simply halving $\Omega_c(t)$ into almost equal segments.
%\begin{algorithm}
%	\caption{Spectrum Partitioning}\label{alg:specpart}
%	\begin{algorithmic}[1]
%		\Procedure{spectrumPartitioning}{}
%		\State \textbf{Initialize:~} $t \gets 0$,~~$c \gets 0$,~~$\Omega_0(0)=\Omega$,~~$C(0)=\{\Omega_0(0)\}$
%		\While{$c<\texttt{length}(C(t))$}													{\color{blue}\Comment{{\scriptsize last region not verified yet}}}
%			\State $\left[Divergenc, u_n\right] \gets \texttt{AdaptiveControl}(\Omega_c(t),u_A)$ 	{\color{blue}\Comment{{\scriptsize verify $\Omega_c(t)$}}}
%			\If{$Divergence = True$} 														{\color{blue}\Comment{{\scriptsize $\Omega_c(t)$ is too wide}}}
%				\State $\left[\Omega^1, \Omega^2\right] \gets \texttt{Divide}(\Omega_c(t))$ {\color{blue}\Comment{{\scriptsize e.g. halve it}}}
%				\State $\Omega_{c+1}(t)\gets \Omega_{c+1}(t)\cup {\Omega^2}$ 				{\color{blue}\Comment{{\scriptsize merge $\Omega^2$ to the next region}}}
%				\State $C(t+1) \gets \left(C(t) - \{\Omega_c(t)\}\right) \cup \{\Omega^1\}$ {\color{blue}\Comment{{\scriptsize replace $\Omega_c(t)$ with a smaller one}}}
%				\State $C(t+1) \gets \texttt{Sort}(C(t+1))$ 								{\color{blue}\Comment{{\scriptsize $\Omega_i(t+1)< \Omega_j(t+1) \Leftrightarrow i<j $}}}
%			\Else 																			{\color{blue}\Comment{{\scriptsize $\Omega_c(t)$ is OK}}}
%				\State $u_A \gets u_n$														{\color{blue}\Comment{{\scriptsize update the feedforward control}}}
%				\State $c \gets c+1$ 														{\color{blue}\Comment{{\scriptsize let's check the next region}}}
%			\EndIf
%			\State $t\gets t+1$ {\color{blue}\Comment{{\scriptsize next iteration}}}
%		\EndWhile\label{euclidendwhile}
%		\EndProcedure
%	\end{algorithmic}
%\end{algorithm}
%\subsection{Band--Pass Filter for Signal to Noise Ratio Improvement}
%As in \eqref{eq:e}, the measurements used in the algorithm are contaminated by broad--band noises. 
%When it comes to compensating for only a segment of the narrow--band disturbances set, a bandpass filter can be utilized in order to decrease the effect of noises at the complementary frequency interval. 
%For instance, if the adaptive compensator is set to compensate harmonics 120 to 150, we would like to minimize the effect of both NRRO and RRO at other frequencies to boost the signal to noise ratio. In that case, the passband of the filter should match the same frequency region. 
%This is discussed in detail and an on--line design method is provided in section~\ref{sec:band-pass filter design}.
